Une version du th\'eor\`eme d'Amer et Brumer pour les z\'ero-cycles

M. Amer and A. Brumer have shown that, for two homogeneous quadratic polynomials f and g in at least 3 variables over a field k of characteristic different from 2, the locus f=g=0 has non-trivial solution over k if and only if, for a variable t, the equation f+tg=0 has a non-trivial solution over k(t). We consider a modified version of this result, and show that the projective variety over k defined by f_0=...=f_r=0, where the f_i are homogeneous polynomials over k of the same degree d\ge2 in n+1 variables (with n+1\ge r+2) , has a 0-cycle of degree 1 over k if and only if the generic hypersurface f_0+t_1f_1+...+t_rf_r=0 has a 0-cycle of degree 1 over k(t_1,...,t_r).

==> CGSS-header.tex <==
%\newcommand{\ack}[1]{\noindent{\small\textbf{Acknowledgements.} {#1}}}
\newcommand{\ack}[1]{\begin{acknowledgement}{#1}\end{acknowledgement}}

\newcommand{\zpar}[1]{\noindent{\textbf{#1} }}

\newcommand{\eand}{\quad\text{and}\quad}

\spnewtheorem{thm}{Theorem}[section]{\bfseries\upshape}{\itshape}
\spnewtheorem{prop}[thm]{Proposition}{\bfseries\upshape}{\itshape}
\spnewtheorem{cor}[thm]{Corollary}{\bfseries\upshape}{\itshape}
\spnewtheorem{lem}[thm]{Lemma}{\bfseries\upshape}{\itshape}
\spnewtheorem{defn}[thm]{Definition}{\bfseries\upshape}{\upshape}
\spnewtheorem{eg}[thm]{Example}{\bfseries\upshape}{\upshape}
\spnewtheorem{rmk}[thm]{Remark}{\itshape}{\upshape}
\spnewtheorem{conj}[thm]{Conjecture}{\bfseries\upshape}{\itshape}
%\spnewtheorem{prop}[thm]{Proposition}{\bfseries\upshape}{\itshape}
\spnewtheorem{egs}[thm]{Examples}{\bfseries\upshape}{\upshape}
\spnewtheorem{ques}[thm]{Question}{\bfseries\upshape}{\itshape}
\spnewtheorem{exer}[thm]{Exercise}{\bfseries\upshape}{\upshape}

\spnewtheorem{degeneration}[thm]{Degeneration}{\bfseries\upshape}{\upshape} 
% for Lieblich
\spnewtheorem{construction}[thm]{Construction}{\bfseries\upshape}{\upshape} 
% for Lieblich
\spnewtheorem{map}[thm]{Map}{\bfseries\upshape}{\upshape} % for Lieblich
\spnewtheorem{sequence}[thm]{Sequence}{\bfseries\upshape}{\upshape} % 
for Lieblich

\spnewtheorem{conjC}[theorem]{Conjecture}{\bfseries\upshape}{\itshape}

% for Skip
\spnewtheorem{borel*}[equation]{}{\bfseries\upshape}{\upshape}

% for Bayer
\spnewtheorem*{thm*}{Theorem}{\bfseries\upshape}{\itshape}

% for Krashen
\spnewtheorem{warn}[thm]{Warning}{\bfseries\upshape}{\upshape}
\spnewtheorem{hyp}[thm]{Hypothesis}{\bfseries\upshape}{\upshape}

% Theorems for Bishnoi-Khanduja
\spnewtheorem*{EIC}{Eisenstein Irreducibility 
Criterion}{\bfseries\upshape}{\itshape}
\spnewtheorem*{DumasCriterion}{Dumas Criterion}{\bfseries\upshape}{\itshape}
\spnewtheorem*{EDKIC}{Eisenstein-Dumas-K\"{u}rsch\'{a}k 
Irreducibility Criterion}{\bfseries\upshape}{\itshape}
\spnewtheorem*{CSIC}{Classical Sch\"onemann Irreducibility 
Criterion}{\bfseries\upshape}{\itshape}
\spnewtheorem*{GSIC}{Generalized Sch\"onemann Irreducibility 
Criterion}{\bfseries\upshape}{\itshape}
\spnewtheorem*{cor*}{Corollary}{\bfseries\upshape}{\itshape}


% Laytimi-Nagaraj
\spnewtheorem*{ques*}{Question}{\bfseries}{\upshape}


\spnewtheorem*{definition*}{Definition}{\bfseries}{\upshape}
\spnewtheorem*{example*}{Example}{\bfseries}{\upshape}
\spnewtheorem*{examples*}{Examples}{\bfseries}{\upshape}
\spnewtheorem*{notation*}{Notation}{\bfseries}{\upshape}
\spnewtheorem*{remark*}{Remark}{\bfseries}{\upshape}
\spnewtheorem*{rmks*}{Remarks}{\bfseries}{\upshape}

\spnewtheorem*{pfidea}{Idea of proof}{\itshape}{\upshape}
\spnewtheorem*{skpf}{Sketch of proof}{\itshape}{\upshape}

\spnewtheorem{propE}[equation]{Proposition}{\bfseries\upshape}{\itshape}
\spnewtheorem{thmE}[equation]{Theorem}{\bfseries\upshape}{\itshape}
\spnewtheorem{lemE}[equation]{Lemma}{\bfseries\upshape}{\itshape}
\spnewtheorem{corE}[equation]{Corollary}{\bfseries\upshape}{\itshape}
\spnewtheorem{conjE}[equation]{Conjecture}{\bfseries\upshape}{\itshape}
\spnewtheorem{egE}[equation]{Example}{\bfseries\upshape}{\upshape}
\spnewtheorem{defnE}[equation]{Definition}{\bfseries\upshape}{\upshape}
\spnewtheorem{rmkE}[equation]{Remark}{\itshape}{\upshape}

\renewcommand{\thetheorem}{\arabic{theorem}}

\setcounter{tocdepth}{0}

\smartqed

%%%%%
%
% Merkurjev
%
%%%%%
\DeclareSymbolFont{operatorsx}{OMX}{cmex}{m}{n}
\DeclareMathSymbol{\dcoprod}{\mathop}{operatorsx}{'141}
\DeclareMathSymbol{\tcoprod}{\mathop}{operatorsx}{'140}


%%%%%
%
% Knus-Tignol
%
%%%%%
  \DeclareMathAlphabet{\cat}{OT1}{cmss}{m}{sl}

  \DeclareMathOperator{\Gal}{Gal}
   \DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\Inv}{Inv}
\DeclareMathOperator{\Int}{Int}
  \DeclareMathOperator{\sgn}{sgn}
% \DeclareMathOperator{\diag}{Diag}
  \DeclareMathOperator{\Iso}{Iso}
  \DeclareMathOperator{\id}{id}
  \DeclareMathOperator{\cont}{cont}
   \DeclareMathOperator{\Hom}{Hom}
   \DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Ext}{Ext}
% \DeclareMathOperator{\disc}{Disc}
  \DeclareMathOperator{\Res}{Res}
  \DeclareMathOperator{\Ker}{Ker}
  \DeclareMathOperator{\Skew}{Skew}
  \DeclareMathOperator{\SSym}{Sym}
   \DeclareMathOperator{\SSymd}{Symd}
  \DeclareMathOperator{\AAlt}{Alt}
  \DeclareMathOperator{\Fix}{Fix}
  \DeclareMathOperator{\Aut}{Aut}
  \DeclareMathOperator{\Out}{Out}
  \DeclareMathOperator{\image}{im}
%  \DeclareMathOperator{\sep}{sep}
  \DeclareMathOperator{\Trd}{Trd}
  \DeclareMathOperator{\Tr}{Tr}
   \DeclareMathOperator{\Map}{Map}
  \DeclareMathOperator{\Nr}{Nr}
  \DeclareMathOperator{\Ind}{Ind}
% \DeclareMathOperator{\op}{op}
  \DeclareMathOperator{\BI}{BI}
  \DeclareMathOperator{\Br}{Br}
\DeclareMathOperator{\carac}{char}
\DeclareMathOperator{\Cycl}{Cycl}
\DeclareMathOperator{\Quadr}{Quad}

\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Mor}{Mor}
\DeclareMathOperator{\im}{im}
